EXION: Exploiting Inter- and Intra-Iteration Output Sparsity for Diffusion Models

Over the past few years, diffusion models have emerged as novel AI solutions, generating diverse multi-modal outputs from text prompts. Despite their capabilities, they face challenges in computing, such as excessive latency and energy consumption due to their iterative architecture. Although prior works specialized in transformer acceleration can be applied, the iterative nature of diffusion models remains unresolved. In this paper, we present EXION, the first SW-HW co-designed diffusion accelerator that solves the computation challenges by exploiting the unique inter- and intra-iteration output sparsity in diffusion models. To this end, we propose two SW-level optimizations. First, we introduce the FFN-Reuse algorithm that identifies and skips redundant computations in FFN layers across different iterations (inter-iteration sparsity). Second, we use a modified eager prediction method that employs two-step leading-one detection to accurately predict the attention score, skipping unnecessary computations within an iteration (intra-iteration sparsity). We also introduce a novel data compaction mechanism named ConMerge, which can enhance HW utilization by condensing and merging sparse matrices into compact forms. Finally, it has a dedicated HW architecture that supports the above sparsity-inducing algorithms, translating high output sparsity into improved energy efficiency and performance. To verify the feasibility of the EXION, we first demonstrate that it has no impact on accuracy in various types of multi-modal diffusion models. We then instantiate EXION in both server- and edge-level settings and compare its performance against GPUs with similar specifications. Our evaluation shows that EXION achieves dramatic improvements in performance and energy efficiency by 3.2-379.3x and 45.1-3067.6x compared to a server GPU and by 42.6-1090.9x and 196.9-4668.2x compared to an edge GPU.

==> Outline/hpca-template.tex <==
\author{
  \ifdefined\hpcacameraready
    \IEEEauthorblockN{\hpcaauthors{}}
      \IEEEauthorblockA{
        \hpcaaffiliation{} \\
        \hpcaemail{}
      }
  \else
    \IEEEauthorblockN{\normalsize{HPCA \hpcayear{} Submission
      \textbf{\#\hpcasubmissionnumber{}}} \\
      \IEEEauthorblockA{
        Confidential Draft \\
        Do NOT Distribute!!
      }
    }
  \fi 
}

% Heading and footer for title page
\fancypagestyle{camerareadyfirstpage}{%
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[C]{
    \ifdefined\aeopen
    \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}    
    \else
      \ifdefined\aereviewed
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \ifdefined\aereproduced
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \parbox[][0mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
    \fi 
    \fi 
    \fi 
    \ifdefined\aeopen 
      \includegraphics[width=12mm,height=12mm]{ae-badges/open-research-objects.pdf}
    \fi 
    \ifdefined\aereviewed
      \includegraphics[width=12mm,height=12mm]{ae-badges/research-objects-reviewed.pdf}
    \fi 
    \ifdefined\aereproduced
      \includegraphics[width=12mm,height=12mm]{ae-badges/results-reproduced.pdf}
    \fi
  }
  %\fancyfoot[L]{\hpcapubid{} \copyright \hpcayear{} IEEE}
  \fancyfoot[C]{}
}
% Heading and footer for remaining pages
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}
%\fancyhead[C]{\hpcayear{} IEEE International Symposium on
% High-Performance Computer Architecture (HPCA)}

==> rebuttal.tex <==
%--------- Consolidated Questions ---------% [TODO] Delete
\textbf{Consolidated Questions=====}

We sincerely thank all the reviewers for their insightful comments. We first addressed the consolidated questions by adding a comparison with Cambricon-D and conducting a sensitivity analysis experiment for FFN-Reuse. Following this, we responded to individual questions and revised the manuscript accordingly.
\newline % [TODO] Delete

(i) Hardware comparison: EXION vs. GPUs

We've added Table II in Section V-B, comparing GPUs to EXION configurations with comparable performance.
\newline % [TODO] Delete

(ii) Comparison with other accelerators

We've added Section V-D to compare the speedup of EXION and Cambricon-D, a SOTA diffusion accelerator, over the NVIDIA A100 GPU. For Stable Diffusion, which includes convolutional layers, Cambricon-D achieves a speedup of 7.9$\times$, slightly exceeding EXION's 7.0$\times$ speedup. However, for the DiT model, which lacks convolutional layers in the denoising iterations, EXION achieves a speedup of 5.2$\times$, outperforming Cambricon-D's 3.3$\times$. Notably, as SOTA image generation models are shifting away from ResBlocks towards transformer-based architectures, Cambricon-D's applicability will be limited. In contrast, EXION's optimizations can be effectively extended to various tasks, such as text- or audio-to-motion generations, where transformer blocks dominate.
\newline % [TODO] Delete

(iii) Sensitivity analysis of FFN-Reuse

The FFN-Reuse algorithm is robust if the hyperparameters, i.e., the threshold for inducing output sparsity and the number of sparse iterations between dense iterations, are not set too aggressively. In other words, the proposed algorithm operates under an accuracy-performance tradeoff rather than being overly sensitive to hyperparameter selection. While the optimal hyperparameter values are statically set for each task based on empirical experiments, the actual sparsity mask is generated at runtime during dense iterations by comparing the FFN's GELU output with the threshold. These approaches have proven sufficient accuracy in our benchmarks, but additional improvement in accuracy is possible with runtime hyperparameter determination (future research).

We further verified that the algorithm performs well with text prompts not included in the original dataset, simulating production environments. We applied FFN-Reuse, EP, and Quantization and tested 100 randomly generated out-of-dataset inputs, achieving robust accuracy. For instance, the measured PSNR values were 17.56dB (MDM) and 24.87dB (Make-an-Audio), compared to 17.67dB and 25.72dB for the original dataset (see Table I), indicating that the output results remain consistent. Figure 16 visualizes one of these outputs, further demonstrating consistent accuracy. This robustness is attributed to our method's ability to leverage inherent similarity across denoising iterations without retraining.
\newline % [TODO] Delete

(iv) Accuracy impact of different optimizations

As verified in Section V-A, our optimizations, such as the FFN-Reuse and EP algorithms, have minimal impact on accuracy. On the other hand, adopting other optimizations, such as token merging and block caching, which have not yet been applied to EXION, may reduce the accuracy of the diffusion model, despite their improvements in computational efficiency.
\newline % [TODO] Delete

%--------------- Reviewer E ---------------% [TODO] Delete
\textbf{Review\#949E=====}

***Separate training set

Our approach does not involve retraining after applying the FFN-Reuse optimization.
\newline % [TODO] Delete

***FFN-Reuse in GPU

FFN-Reuse originates as a SW-level optimization, but the resulting output sparsity is highly unstructured, making it difficult for GPUs to accelerate efficiently. While condensing can be applied, its effect remains limited in models like Stable Diffusion, DiT, and VideoCrafter2 (see Section V-C). Additionally, GPUs incur latency overhead in checking whether all elements in each column are sparse for condensing. In contrast, EXION hides all of this latency through CAU support and efficient scheduling.
\newline % [TODO] Delete

***Command for data reuse

While hyperparameters are set statically, control signals that are generated with the sparsity mask and partial sums of sparse data are produced at runtime during dense iterations for each input (see Figure 6). EXION's ISA includes a reuse command that leverages these control signals and partial sums to instruct EXION to compute only non-sparse data and accumulate it into partial sums during sparse iterations.
\newline % [TODO] Delete

%--------------- Reviewer C ---------------% [TODO] Delete
\textbf{Review\#949C=====}

***Statement in introduction

The energy consumption and latency values for Stable Diffusion and StyleGAN-XL were measured directly by us under identical conditions using the same GPU device, rather than being referenced from other works.
\newline % [TODO] Delete

***Block merging in detail

We've added Figure 14 and provided additional explanations in Section IV-C to clarify how the column information is retained during merging.
\newline % [TODO] Delete

%--------------- Reviewer B ---------------% [TODO] Delete
\textbf{Review\#949B=====}

***Merging algorithm and specialized HW

We've added explanations and Figure 14 to provide details on how the algorithm is implemented and how control signals are generated.
\newline % [TODO] Delete

***Restoring matrix after calculation

The matrix does not need to be restored across iterations, as it is already restored within each iteration for further computations. During a dense iteration, EXION generates ConMerge vectors and stores them in CVMEM. In subsequent sparse iterations, it performs MMUL on the condensed and merged matrix using these vectors. EXION processes computations in tiled units, tailored to SDUE hardware. Once DSC's output memory is full, it transfers data to the GSC, which has a data aligner. While DSC continues processing the next tiles, the data aligner in GSC concurrently restores the matrix for the next computation in DSC by using control signals stored in CVMEM.
\newline % [TODO] Delete

***Inference framework's modification

At a high-level abstraction, no modifications are needed. However, as EXION uses its own ISA, the compiler requires updates to support these specific instructions.
\newline % [TODO] Delete

***Hyperparameter selection

The hyperparameters of FFN-Reuse are selected based on an accuracy-performance tradeoff. We chose values that maximize acceleration opportunities without compromising accuracy.
\newline % [TODO] Delete

***Memory bank configuration

The number of banks in IMEM and WMEM aligns with the rows and columns of the DPU array, respectively, to simply and efficiently broadcast data. This configuration is fixed based on the tiled unit size and cannot be adjusted by software.
\newline % [TODO] Delete

%--------------- Reviewer A ---------------% [TODO] Delete
\textbf{Review\#949A=====}

***Multimodal scenarios

As described in Table I, EXION can handle various multimodal scenarios by running transformer-based conditioning networks, such as CLIP and CLAP, to transform inputs (e.g., text and sound) into embeddings. These embeddings are then integrated into the diffusion network during its denoising steps, allowing the generated output to accurately reflect the provided inputs.
